Link Recommendation to Augment Influence Diffusion with Provable Guarantees

Link recommendation systems in online social networks (OSNs), such as Facebook's ``People You May Know'', Twitter's ``Who to Follow'', and Instagram's ``Suggested Accounts'', facilitate the formation of new connections among users. This paper addresses the challenge of link recommendation for the purpose of social influence maximization. In particular, given a graph $G$ and the seed set $S$, our objective is to select $k$ edges that connect seed nodes and ordinary nodes to optimize the influence dissemination of the seed set. This problem, referred to as influence maximization with augmentation (IMA), has been proven to be NP-hard. In this paper, we propose an algorithm, namely \textsf{AIS}, consisting of an efficient estimator for augmented influence estimation and an accelerated sampling approach. \textsf{AIS} provides a $(1-1/\mathrm{e}-\varepsilon)$-approximate solution with a high probability of $1-\delta$, and runs in $O(k^2 (m+n) \log (n / \delta) / \varepsilon^2 + k \left|E_{\mathcal{C}}\right|)$ time assuming that the influence of any singleton node is smaller than that of the seed set. To the best of our knowledge, this is the first algorithm that can be implemented on large graphs containing millions of nodes while preserving strong theoretical guarantees. We conduct extensive experiments to demonstrate the effectiveness and efficiency of our proposed algorithm.

==> figures/_tex/fig_rr_set_as_cover.tex <==
\begin{figure}[H]
    \centering
    \includesvg[scale=0.9]{figures/IM_cover.svg}
    % \includegraphics[scale=0.4]{figures/rrset_cover.png}
    \caption{Illustration of connecting RIS and maximum coverage problem.}
    \label{fig:ris_cover}
\end{figure}

==> figures/include_files/mcg_time_r_grqc_nethept.tex <==
\begin{figure}[!t]
\centering
\begin{small}
% \begin{tikzpicture}
%     \begin{customlegend}[legend columns=2,
%         legend entries={$\mathsf{AIS}$, $\mathsf{MC-greedy}$},
%         legend style={at={(0.45,1.35)},anchor=north,draw=none,font=\footnotesize,column sep=0.15cm}]
%     \addlegendimage{smooth,color=red,mark=triangle, mark size=3}
%     \addlegendimage{smooth,mark=asterisk,color=XL4}
%     \end{customlegend}
% \end{tikzpicture}
% \\[-\lineskip]
% \vspace{-1mm}
\subfloat[{\em GRQC}]{
\includegraphics{figures/mcg_time_r_grqc.pdf}
}%
\subfloat[{\em NetHEPT}]{
\includegraphics{figures/mcg_time_r_nethept.pdf}
}%

\vspace{-3mm}
\end{small}
\caption{Running Time (sec) v.s. $r$ on GRQC and NetHEPT} \label{fig:mcg_time_r}
\vspace{-2mm}
\end{figure}

==> sections/algo/IMA_IC.tex <==
\begin{algorithm}
\caption{\texttt{AIS}}\label{alg:IMA}

\begin{algorithmic}[1]
\Require $\mathcal{R}, k, E_\candidates$
\Ensure Top-$k$ edges
\State $A_k \gets \emptyset$
\State $\rrsets \gets \texttt{Sampling}(G, k, \varepsilon, \delta)$
\For{$i=1$ to $k$}
    \State $e^* \gets \operatorname*{arg\,max}\limits_{\anglePair{u,v}} p_{u, v} \cdot (\covSets{\rrsets}{S\cup \{v\}} - \covSets{\rrsets}{S})$
    \State $E_\candidates \gets E_\candidates \bksls e^*$
    \State $A_k \gets A_k \cup \{e^*\}$
    \State \texttt{Augment}($\rrsets$, $e^*$)
\EndFor
\State \Return $A_k$
\end{algorithmic}
\end{algorithm}

==> sections/algo/IMA_IC_acc.tex <==
\begin{algorithm}
\caption{\ais}\label{alg:AIS}

\begin{algorithmic}[1]
\Require $\mathcal{R}, S, k, E_\candidates, \varepsilon, \delta$
\Ensure Edge set $A$
\State $\eta \gets \min{\{\abs{\Ecand}, n\}}$
\State $\rrsets \gets \texttt{Sampling}(G, k, \frac{\varepsilon / k}{2 + \varepsilon / k}, \frac{\delta}{2\eta} )$
\State \Return $\texttt{EdgeSelection}(\rrsets, k, \Ecand)$
\end{algorithmic}
\end{algorithm}

==> sections/algo/alg_IMM_sample.tex <==
\begin{algorithm}
\caption{\texttt{Sampling}}\label{alg:IMM_sample}

\begin{algorithmic}[1]
\Require $G$, $\varepsilon$, $k$, $\delta$
\Ensure $\rrsets$

\State $\rrsets \gets \emptyset, \text{LB} \gets 1, \delta \gets \delta / \log_2 n$
\State $\gamma \gets \frac{(2 + \frac{2}{3} \varepsilon)\log (1/\delta)}{\varepsilon^{2}}
    \cdot n$

\For{$i=1$ to $\log_2 n - 1$}
    \State $x \gets n/2^i$
    \State $\theta_i \gets \gamma / x$
    \While{$\abs{\rrsets} \leq \theta_i$}
        \State $R \gets$ Sample a random RR set
        \State $\rrsets \gets \rrsets \cup \{R\}$
    \EndWhile
    \If{$n\cdot F_{\rrsets}(S) \geq (1 + \varepsilon)\cdot x$}
        % \State $\text{LB} = n\cdot F_{\rrsets}(S) / (1 + \varepsilon)$
        \State \textbf{break};
    \EndIf
\EndFor
% \State $\theta \gets \gamma / \text{LB}$
% \While{$\abs{\rrsets} \leq \theta$}
%     \State $R \gets \texttt{GetRandomRRset}(G)$
%     \State $\rrsets \gets \rrsets \cup \{R\}$
% \EndWhile
\State \Return $\rrsets$

\end{algorithmic}
\end{algorithm}

==> sections/algo/alg_sampling.tex <==
\begin{algorithm}
\caption{\texttt{Sampling}}\label{alg:sample_stopping_rule}

\begin{algorithmic}[1]
\Require $G$, $\lambda$, $\delta$
\Ensure $\rrsets$

\State $\rrsets \gets \emptyset$, $\theta \gets 0$, $\Sigma \gets 0$
\State $\Upsilon \gets \frac{2(1+\lambda)(1 + \frac{\lambda}{3})\log (2/\delta)}{\lambda^{2}}$

\While{$\Sigma < \Upsilon$}
    \State $R \gets$ Sample a random RR set
    \State $\rrsets \gets \rrsets \cup \{R\}$
    \State $\theta \gets \theta + 1$
    \If{$R$ is covered by $S$}
    \State $\Sigma \gets \Sigma + 1$
    \EndIf
\EndWhile
\State \Return $\rrsets$

\end{algorithmic}
\end{algorithm}

==> sections/algo/comp_marginal_gain.tex <==
\begin{algorithm}
\caption{\texttt{CompMarginalGain}}\label{alg:node_selection}

\begin{algorithmic}[1]
\Require $\mathcal{R}, k$
\Ensure An array of the marginal gains of all edges in $E_\candidates$.
\State $S_k \gets \emptyset$ 
\For{$i=1$ to $k$}
    \State $v \gets \operatorname*{arg\,max}\limits_u F_{\mathcal{R}}(S \cup \{u\}) - F_{\mathcal{R}}(S)$
    \State $S_k \gets S_k \cup \{v\}$
\EndFor

\State \Return $S_k$

\end{algorithmic}
\end{algorithm}

==> sections/algo/edge_selection.tex <==
\begin{algorithm}
\caption{\texttt{EdgeSelection}}\label{alg:edge_selection}

\begin{algorithmic}[1]
\Require $\mathcal{R}, k, S, \Ecand$
\Ensure An edge set $A$ with size $k$
\State $A \gets \emptyset$ 
\For{$v$ in $S$}    \label{alg:edge_selection_init_begin}
    \For{$R$ in the RR sets covered by $v$}
        \State \text{cov\_by\_S}[R] $\gets$ true
    \EndFor
\EndFor
\For{$v$ in $V$}
    \For{$R$ in the RR sets covered by $v$}
        \If{\text{cov\_by\_S}[R] == false}
            \State m\_cov[$v$]++    \label{alg:edge_selection_init_end}
        \EndIf
    \EndFor
\EndFor
\For{$i=1$ to $k$}
    \State $e^* \gets \operatorname*{arg\,max}\limits_{\anglePair{u,v,\puv} \in \Ecand \bksls A} p_{u, v} \cdot \text{m\_cov}[v]$ \label{eq:marg_gain_in_code}
    \State $A \gets A \cup \{e^*\}$
    \State $\anglePair{u,v,\puv} \gets e^*$
    \For{$R$ in the RR sets covered by $v$} \label{alg:edge_selection_update_begin}
        \If{cov\_by\_S[$R$]}
            \State \textbf{continue}
        \EndIf
        \If{$\texttt{rand()} \leq \puv$}
            \State cov\_by\_S[$R$] $\gets$ true
            \For{$z$ in $R$}
                \State m\_cov[$z$]$--$  \label{alg:edge_selection_update_end}
            \EndFor
        \EndIf
    \EndFor
\EndFor
\State \Return $A$

\end{algorithmic}
\end{algorithm}

==> sections/algo/get_rand_rrset.tex <==
\begin{algorithm}
\caption{\texttt{GetRandomRRset}}\label{alg:randRRset}
\begin{algorithmic}[1]
\Require $G$
\Ensure $R$
\State Select a node $u$ from $G$ uniformly at random.
\State Generate a RR set $R$ from node $u$.
\State \Return $R$
\end{algorithmic}
\end{algorithm}

==> sections/algo/node_select.tex <==
\begin{algorithm}
\caption{\texttt{NodeSelection}}\label{alg:node_selection}

\begin{algorithmic}[1]
\Require $\mathcal{R}, k$
\Ensure A seed set $S_k$ with size $k$
\State $S_k \gets \emptyset$ 
\For{$i=1$ to $k$}
    \State $v \gets \operatorname*{arg\,max}\limits_u F_{\mathcal{R}}(S \cup \{u\}) - F_{\mathcal{R}}(S)$
    \State $S_k \gets S_k \cup \{v\}$
\EndFor

\State \Return $S_k$

\end{algorithmic}
\end{algorithm}

==> sections/lemmas/lem_1.tex <==
\begin{lemma}
\label{lem:1}
For any $\delta^\prime \geq 1$, pick $\frac{6\delta^\prime}{\varepsilon^2 \text{Opt}_k}\leq p \leq 1$, and let $S$ be an arbitrary subset of $V$ s.t. $|S|\leq k$. With probability $1-e^{-\delta^\prime}$, we have
\begin{equation}
\label{eq:FR_est}
    \left| \frac{1}{p}\Lambda_{\mathcal{R}_p}(S) - \Lambda_{\mathcal{R}}(S) \right| \leq \varepsilon \text{Opt}_k
\end{equation}
\end{lemma}
\textit{Proof: } Let $X_i$ be a r.v indicating whether $R_i$ is abandoned or not. That is, $X_i = 1$ if $h(R_i)\leq p$, 0 otherwise. Then we have
\begin{equation}
    \sum_{i=1}^{\Lambda_{\mathcal{R}}(S)} X_i = \Lambda_{\mathcal{R}_p}(S)
\end{equation}

\begin{equation}
    \mathbb{E}[\sum_{i=1}^{\Lambda_{\mathcal{R}}(S)} X_i] = \sum_{i=1}^{\Lambda_{\mathcal{R}}(S)} \mathbb{E}[X_i] = p\Lambda_{\mathcal{R}}(S).
\end{equation}

Inspired by Chernoff bounds,
\begin{equation}
    \begin{aligned}
    &\Pr\left[\left|\sum_{i=1}^{\Lambda_{\mathcal{R}}(S)} X_i - \mathbb{E}[\sum_{i=1}^{\Lambda_{\mathcal{R}}(S)} X_i]\right| \geq \varepsilon^\prime \mathbb{E}[\sum_{i=1}^{\Lambda_{\mathcal{R}}(S)} X_i]\right]\\
    &=\Pr[|\Lambda_{\mathcal{R}_p}(S) - p\Lambda_{\mathcal{R}}(S)|\geq \varepsilon^\prime p \Lambda_{\mathcal{R}}(S)]\\
    &\leq 2\exp \left[\frac{-{\varepsilon^\prime}^2 p \Lambda_{\mathcal{R}}(S)}{3}\right]\\
    \end{aligned}
\end{equation}
Let $\varepsilon^\prime = \varepsilon\cdot \frac{\text{Opt}_k}{\Lambda_{\mathcal{R}}(S)}$,
\begin{equation}
    \begin{aligned}
    &\Pr
    \left[
    |\Lambda_{\mathcal{R}_p}(S) - p\Lambda_{\mathcal{R}}(S)|\geq 
    \varepsilon p \text{Opt}_k
    \right]\\
    &\leq 2\exp \left(
    \frac{-\varepsilon^2 \frac{\text{Opt}_k^2}{\Lambda_{\mathcal{R}}^2(S)} 
    p \Lambda_{\mathcal{R}}(S)}{3}
    \right)\\
    &= 2\exp \left(-\frac{p\varepsilon^2 \text{Opt}_k^2}{3\Lambda_{\mathcal{R}}(S)}
    \right)\\
    &= 2\exp \left(
    -\frac{6\delta^\prime}{\varepsilon^2 \text{Opt}_k}
    \cdot
    \frac{\varepsilon^2 \text{Opt}_k^2}{3\Lambda_{\mathcal{R}}(S)}
    \right)\\
    &= 2\exp \left(
    -\frac{2\delta^\prime \text{Opt}_k}{\Lambda_{\mathcal{R}}(S)}
    \right)\\
    &\leq 2\exp \left(
    -2\delta^\prime
    \right)\\
    &\leq \exp \left(
    1 - 2\delta^\prime
    \right)\\
    &\leq \exp \left(
    -\delta^\prime
    \right).\\
    \end{aligned}
\end{equation}
Then,
\begin{equation}
    \begin{aligned}
    &\Pr
    \left[
    \left|\Lambda_{\mathcal{R}_p}(S) - p\Lambda_{\mathcal{R}}(S)\right|
    \leq 
    \varepsilon p \text{Opt}_k
    \right]\\
    &\geq 1 - \exp \left(
    -\delta^\prime
    \right)
    \end{aligned}
\end{equation}

% Next we find the way to express the inequality by $F_\mathcal{R}(S)$.
% \begin{equation}
%     \begin{aligned}
%     &\Pr \left[
%     |\Lambda_{\mathcal{R}_p}(S) - p\Lambda_{\mathcal{R}}(S)|\leq 
%     \varepsilon p \text{Opt}_k
%     \right]
%     \\
%     &= \Pr \left[
%     \left|
%     \frac{1}{p}
%     \Lambda_{\mathcal{R}_p}(S) - \Lambda_{\mathcal{R}}(S) 
%     \right|
%     \leq 
%     \varepsilon \text{Opt}_k
%     \right]\\
%     &= \Pr \left[
%     \left|
%     \frac{1}{p\theta}
%     \Lambda_{\mathcal{R}_p}(S) - \frac{1}{\theta} \Lambda_{\mathcal{R}}(S) 
%     \right|
%     \leq 
%     \varepsilon \frac{\text{Opt}_k}{\theta}
%     \right]\\
%     &= \Pr \left[
%     \left|
%     \frac{1}{\theta_p}
%     \Lambda_{\mathcal{R}_p}(S) - \frac{1}{\theta} \Lambda_{\mathcal{R}}(S) 
%     \right|
%     \leq 
%     \varepsilon \frac{\text{Opt}_k}{\theta}
%     \right]\\
%     &= \Pr \left[
%     \left|
%     F_{\mathcal{R}_p}(S) - F_{\mathcal{R}}(S) 
%     \right|
%     \leq 
%     \varepsilon \frac{\text{Opt}_k}{\theta}
%     \right]\\
%     \end{aligned}
% \end{equation}
That is,
\begin{equation}
    \Pr
    \left[
    \left|\frac{1}{p}\Lambda_{\mathcal{R}_p}(S) - \Lambda_{\mathcal{R}}(S)\right| \leq 
    \varepsilon \text{Opt}_k
    \right]
    \geq 1-e^{-\delta^\prime}
\end{equation}



==> sections/lemmas/lem_EPT.tex <==
\begin{lemma}[\cite{tang2014influence}]\label{lem:AVG}
    Use $\AVG$ to denote the expected number of coin tosses required to generate an RR set and $v^*$ is a random node following the probability distribution where the probability for selecting each node is proportional to its in-degree. We have
    \begin{equation}
        \AVG = \frac{m}{n} \expect{\sigma (\{v^*\})},
    \end{equation}
    where the expectation is taken over the randomness of $v^*$.
\end{lemma}

==> sections/lemmas/lem_IMM_sample_1.tex <==
\begin{lemma}
\label{lem:IMM_sample_1}
Let $x\in [1, n]$, and $\varepsilon, \delta \in (0, 1)$. Suppose that we sample a set $\rrsets$ containing $\theta$ RR sets, with:
\begin{equation}
\label{eq:sample_1}
    \theta \geq \frac{(2 + \frac{2}{3} \varepsilon)\log (1/\delta_2)}{\varepsilon^{2}}
    \cdot \frac{n}{x}.
\end{equation}
If $\sigma(S) < x$, we have $n\cdot F_{\rrsets} (S) < (1 + \varepsilon) \cdot x$ with at least $1 - \delta_2$ probability.
\end{lemma}

\begin{proof}
    Use $x_i$ to denote the random variable such that for each RR set $R_i \in \rrsets$, $x_i=1$ if $S\cap R_i \neq \emptyset$, and $x_i=0$ otherwise. Define $p$ as follows,
    \begin{equation}
        p = \expect{\fracR{\rrsets}{S}} = \sigma(S) / n < x / n.
    \end{equation}
    Let $\xi = \frac{(1+\varepsilon)x}{np} - 1$.
    \begin{equation}
        \begin{aligned}
            &\Pr[n \fracR{\rrsets}{S} \geq (1+\varepsilon)x]\\
            =& \Pr[\theta \fracR{\rrsets}{S} \geq \frac{(1+\varepsilon)x}{n}\cdot \theta]\\
            =& \Pr[\theta \fracR{\rrsets}{S} - \theta p \geq (\frac{(1+\varepsilon)x}{np} - 1) \cdot \theta p]\\
            \leq& \exp \left(
            -\frac{\xi^2}{2 + 2\xi / 3} \cdot \theta p
            \right)\\
            <& \exp \left(
            -\frac{\varepsilon \cdot x / (np)}{2/\xi + 2 / 3} \cdot \frac{(2 + \frac{2}{3} \varepsilon)\log (1/\delta_2)}{\varepsilon^{2}} \cdot \frac{np}{x}
            \right)\\
            <& \exp \left(
            -\frac{\varepsilon \cdot x / (np)}{2/\varepsilon + 2 / 3} \cdot \frac{(2 + \frac{2}{3} \varepsilon)\log (1/\delta_2)}{\varepsilon^{2}} \cdot \frac{np}{x}
            \right)\\
            <& \delta_2.
        \end{aligned}
    \end{equation}
    The proof is complete.
\end{proof}

==> sections/lemmas/lem_IMM_sample_2.tex <==
\begin{lemma}
\label{lem:IMM_sample_2}
If $\sigma(S) \geq x$, then we have $\sigma(S) \geq n\cdot F_{\rrsets} (S) / (1 + \varepsilon^\prime)$ with probability at least $1 - \delta_2$.
\end{lemma}

\begin{proof}
    \begin{equation}
        \begin{aligned}
            \Pr[\sigma(S) < n F_{\rrsets} (S) / (1 + \varepsilon^\prime)] =& \Pr[n \fracR{\rrsets}{S} > (1+\varepsilon^\prime)\sigma (S)]\\
            =& \Pr[\theta \fracR{\rrsets}{S} > (1+\varepsilon^\prime)\theta p]\\
            =& \Pr[\theta \fracR{\rrsets}{S} - \theta p > \varepsilon^\prime\theta p]\\
            \leq& \exp \Brackets{
            -\frac{\varepsilon^{\prime 2}}{2 + 2\varepsilon^\prime /3} \cdot \theta p
            }\\
            =& \exp \Brackets{
            - (\sigma (S) / x) \cdot \log (1/\delta_2)
            }\\
            \leq& \delta_2
        \end{aligned}
    \end{equation}
\end{proof}

==> sections/lemmas/lem_IMM_sample_3.tex <==
\begin{lemma}\label{lem:IMM_sample_3}
    If $\sigma(S) \geq c \cdot (1+\varepsilon^\prime)^2 x$, then $n\cdot \fracR{\rrsets}{S}\leq (1+\varepsilon^\prime)x$ holds with at most $(\delta_2)^c$ probability.
\end{lemma}

\begin{proof}
Let $p=\sigma (S) / n$ and $\xi = \frac{\varepsilon^\prime}{1 + \varepsilon^\prime}$.
    \begin{equation}
        \begin{aligned}
            \Pr [n\fracR{\rrsets}{S} \leq (1+\varepsilon^\prime)x] =& \Pr [\theta \fracR{\rrsets}{S} \leq (1+\varepsilon^\prime)\frac{x}{n} \theta]\\
            \leq& \Pr [\theta \fracR{\rrsets}{S} \leq \frac{1}{1+\varepsilon^\prime} \theta p]\\
            =& \Pr [\theta \fracR{\rrsets}{S} - \theta p \leq -\xi \theta p]\\
            \leq& \exp \Brackets{-\frac{\xi}{2}\theta p}\\
            <& (\delta_2)^c
        \end{aligned}
    \end{equation}
\end{proof}

==> sections/lemmas/lem_IMM_sample_4.tex <==
\begin{lemma}\label{lem:LB_lower_bound}
    Let $\rrsets$ be the output of Algorithm \ref{alg:IMM_sample}. We have $x \geq \frac{\sigma (S)}{(1+\varepsilon)^2}$ with probability at least $1-\delta_2$.
\end{lemma}

\begin{proof}
    Assume that $\sigma (S) \geq (1+\varepsilon)^2 x$ first holds in the $j$-th iteration. Let $z \geq j$. In the $z$-th iteration, we have $\sigma(S) \geq 2^{z-j} \cdot (1+\varepsilon)^2 \cdot \frac{n}{2^z}$. Use $I_z$ to denote the event that we reach the $z$-th iteration in the for loop. By Lemma \ref{lem:IMM_sample_3}, we know that $\Pr [I_z] \leq \delta_2 / \log_2 n$. Since the total number of iterations is bounded by $\log_2 n$, by the union bound, Algorithm \ref{alg:IMM_sample} terminates in the $j$-th iteration with at least $1-\delta_2$ probability, where $\sigma (S) \leq (1+\varepsilon)^2 x$. Finally, we have
    \begin{equation}
        x_{j-1} = 2 x_j \geq \frac{\sigma(S)}{(1+\varepsilon)^2}
    \end{equation}
    
    Hence we have $x_j \geq \frac{\sigma(S)}{2(1+\varepsilon)^2}$. The lemma is proved.
\end{proof}

==> sections/lemmas/lem_bounds_of_theta.tex <==
\begin{lemma}\label{lem:bounds_theta}
    Let $\rrsets$ be the RR sets returned by Algorithm \ref{alg:sample_stopping_rule}. If $(1-\lambda)\sigma (S) \leq n\fracR{\rrsets}{S} \leq (1+\lambda)\sigma (S)$, we have
    \begin{equation}
         \frac{\myceil{\Upsilon}}{(1+\lambda)\sigma (S)} \leq \theta \leq \frac{\myceil{\Upsilon}}{(1-\lambda)\sigma (S)}
    \end{equation}
\end{lemma}

==> sections/lemmas/lem_estimation_all_rounds.tex <==
\begin{lemma}\label{lem:lambda_err_for_all}
Let $\rrsets$ be the RR sets sampled by \ref{alg:AIS}.
% Suppose the number of RR sets $\theta$ satisfies
% \begin{equation}\label{eq:rrset_num_union_bound}
%     \theta > \frac{(2 + \frac{2}{3}\lambda)n \log (2k \eta/\delta)}{\sigma(S) \lambda^2}.
% \end{equation}
With probability at least $1-\delta$, it holds for all iterations of Algorithm \ref{alg:edge_selection} that $\forall e = \anglePair{u, v} \in \Ecand$,
\begin{equation}
    (1-\lambda) \mu(A \cup \{e\}) \leq \hat{\mu}(A \cup \{e\}) \leq (1+\lambda) \mu (A \cup \{e\}).
\end{equation}

\end{lemma}

\begin{proof}
    From Theorem \ref{thm:stopping_rule}, we can easily show that if in the first iteration where no edge is added into the network, $n\fracR{\rrsets}{S}$ provides a $(\lambda, \frac{\delta}{k \eta})$-estimate of $\sigma(S)$, then we can claim that after adding edges $A$ to the network, the number of RR sets is still enough to give a $(\lambda, \frac{\delta}{k\eta})$-estimate of the spread of $S$. This is intuitive since the function $\sigma (\cdot, S)$ is monotone. When we have a enough samples to estimate a smaller value with a multiplicative error, then the number of samples is also enough to estimate a larger value with the same error.
    
    Now we investigate how many estimations we need to make in total. We need to select $k$ edges overall, so the algorithm runs for $k$ rounds. In every round, we need to compute the marginal gain of every candidate edge. For one candidate edge $\anglePair{u,v,\puv}$, we need to estimate $\sigma(A\cup \{e\}, S)$, which is equivalent to estimating $\sigma(A, S \cup \{v\})$ according to Lemma \ref{lem:link_marginal_gain}. Notice that the number of different nodes is at most $\min{ \{\abs{\Ecand}, n\} }$. Thus, there are $k\min{ \{\abs{\Ecand}, n\} }$ different estimations in total. So by the union bound, with probability at least $1-\delta$, it holds for every iteration that
    \begin{equation}\label{eq:lambda_est}
        (1-\lambda)\sigma (A, S) \leq n\fracR{\rrsets}{S} \leq (1+\lambda) \sigma (A, S).
    \end{equation}

    Then we look into one iteration. In every iteration, we want to select the edge from the candidate edge set that results in largest $\mu (A \cup \{e\})$. Conditioning on (\ref{eq:lambda_est}), we will show that $\hat{\mu} (A \cup \{e\})$ is a $\lambda$-estimate of $\mu (A \cup \{e\})$.
    \begin{equation}
        \begin{aligned}
            \hat{\mu} (A \cup \{e\}) &= n(\fracR{\rrsets}{S} - \puv \fracR{\rrsets}{v|S})\\
            &= n (1-\puv) \fracR{\rrsets}{S} + n\puv \fracR{\rrsets}{S \cup \{v\}}\\
            &\leq (1+\lambda)((1-\puv)\sigma (A, S) + \puv \sigma (A, S \cup \{v\}))\\
            &= (1+\lambda) \mu (A \cup \{e\}).
        \end{aligned}
    \end{equation}
    Following the same manner, we can easily prove that $\hat{\mu} (A\cup \{e\}) \geq (1-\lambda) \mu (A\cup \{e\})$. Hence the proof is finished.
    % Use $A_i$ to denote the event $n\fracR{\rrsets}{S}$ fails bound the error within $\lambda$ for the $i$-th estimation, and $B$ to denote the event that at least one estimation fails. Since $\Pr[A_i] \leq \frac{\delta}{\eta}$ holds for all $i$, then by the union bound,
    % \begin{equation*}
    %     \Pr[B] = \Pr \left[{\textstyle \bigcup_{i}} A_i \right] \leq \sum_{i} \Pr[A_i] \leq \delta.
    % \end{equation*}
    % Therefore, with probability at least $1-\delta$, it holds that $n\fracR{\rrsets}{S}$ gives a $\lambda$-estimate of the spread of $S$ in every iteration. Hence the proof is finished.
\end{proof}

==> sections/lemmas/lem_frac_opt.tex <==
\begin{lemma} [\cite{tang2014influence}]
\label{lem:frac_opt}
    Setting
    \begin{equation}
    \label{eq:params}
        \begin{aligned}
        \alpha &= \sqrt{l\log n + \log 2}\\
        \beta &= \sqrt{(1-1/e) \cdot (\log {\textstyle \binom{n}{k}} + l\log n + \log 2)}\\
        \lambda^* &= \frac{2n\cdot ((1-1/e)\cdot \alpha + \beta)^2}{\varepsilon_0^2},
        \end{aligned}
    \end{equation}
    and given a $\theta$ satisfying
    \begin{equation}
        \theta \geq \frac{\lambda^*}{\OPT},
    \end{equation}
    for any set $S$ of at most $k$ nodes, the following inequality holds with probability at least $1 - n^{-l} / {n \choose k}$.
    \begin{equation}
    \label{eq:frac_inf}
        \left| n\frac{\covSetsNum{\rrsets}{S}}{\theta} - \sigma(S) \right| \leq \frac{\varepsilon_0}{2}OPT
    \end{equation}
\end{lemma}

==> sections/lemmas/lem_num_RRsets.tex <==
\begin{lemma}\label{lem:single_est}
    Let $\delta_1 \in (0,1)$, $\lambda > 0$, and
    \begin{equation}\label{eq:rrset_num}
        \theta > \frac{(2 + \frac{2}{3}\lambda)n \log (2/\delta_1)}{\sigma(S) \lambda^2}.
    \end{equation}
    $n\covSets{\rrsets}{S} / \theta$ is a $(\lambda, \delta_1)$-estimation of $\sigma(S)$.
\end{lemma}

\begin{proof}
    By utilizing the martingale concentration inequalities,
    \begin{equation}
        \begin{aligned}
            \Pr[n \fracR{\rrsets}{S} \geq (1+\lambda)\sigma(S)]
            =& \Pr[n \fracR{\rrsets}{S} \geq (1+\lambda)\sigma(S)]\\
            =& \Pr[n \fracR{\rrsets}{S} \geq (1+\lambda)np]\\
            =& \Pr[\theta \fracR{\rrsets}{S} \geq (1+\lambda)\theta p]\\
            =& \Pr[\theta \fracR{\rrsets}{S} - \theta p \geq \lambda \theta p]\\
            \leq& \exp \left(-\frac{\lambda^2}{2 + \frac{2}{3}\lambda} \theta p \right)\\
            \leq& \exp \left(-\log (2/\delta_1) \right) = \delta_1 / 2.
        \end{aligned}
    \end{equation}
    Similarly,
    \begin{equation}
        \begin{aligned}
            \Pr[n\fracR{\rrsets}{S} \leq (1-\lambda) \sigma(S)] 
            =& \Pr[\theta \fracR{\rrsets}{S} - \theta p \leq -\lambda \theta p]\\
            \leq& \exp \left( -\frac{\lambda^2}{2} \theta p \right)\\
            =&  \exp \left( -\frac{\lambda^2}{2} \frac{2+\frac{2}{3}\lambda}{\lambda^2}\log (2/\delta_1) \right)\\
            <& \delta_1 / 2.
        \end{aligned}
    \end{equation}
\end{proof}

==> sections/lemmas/lem_rrset_aug_time.tex <==
\begin{lemma}\label{lem:rrset_update_time}
    Let $v^\circ$ be the most influential node in the network. The time complexity of the RR set update process is bounded by $O(\frac{k^3\log (kn /\delta)}{\varepsilon^{2}} \cdot \frac{\sigma(\{v^\circ\})}{\sigma(S)})$.
\end{lemma}

\begin{proof}
We break the RR sets update process into two parts, check and modify. Every time an edge $e = \anglePair{u, v}$ is selected, we first need to traverse all RR sets containing $v$, which costs $O(\covSets{\rrsets}{\{v\}})$. Then, for each RR set $R$ containing $v$, we check if $e$ is alive in this probability world. If $e$ is alive, the marginal coverage values of all nodes in $R$ will decrease by $1$.

To start with the easy part, we first show that the modify part costs at most $O(\sum \abs{R})$. If the addition of $e$ lets $S$ successfully cover a RR set $R$, the algorithm will traverse all nodes in $R$ and update their marginal coverage, which costs $O(\abs{R})$. Also, notice that once a RR set is covered by $S$, we will not traverse it again. So the time complexity for the modify part is at most $O(\sum \abs{R})$.

Then we look into the check part. As the checking operation will be conducted every time we add a new edge into our solution set, the time complexity could be written as $O(\sum_{e\in A_k} \covSets{\rrsets}{\{v\}})$. A special case is each edge in $A_k$ has different target node from others. Namely we only recommend one seed node to an ordinary node. In this scenario, the time complexity is bounded by $O(\sum \abs{R})$. If we select $k$ edges from a candidate set with size $O(k_0 n)$, the special case is likely to happen. However, to bound the time complexity for more general situations, we need to carry out more detailed analysis.

\begin{equation}
    \sum_{e \in A_k} \covSets{\rrsets}{\{v\}} = O(\frac{\theta}{n} \sum_{e \in A_k} \sigma(\{v\}) ) \leq  O(\frac{\theta}{n} k\sigma(\{v^\circ\}) )
\end{equation}
Therefore, the total time complexity of RR sets update process is $O(\frac{k^3 \log (kn / \delta)}{\varepsilon^2} \cdot \frac{\sigma(\{v^\circ\})}{\sigma(S)})$.
\end{proof}

==> sections/lemmas/lem_sample_1.tex <==
\begin{theorem}
\label{lem:sample_1}
Let $x\in [0, 1]$, and $\varepsilon^\prime, \delta \in (0, 1)$. Suppose that we implement Algorithm \ref{alg:node_selection} on a set $\rrsetsCon$ containing $\theta$ random size-constrained RR sets, with equation \ref{eq:sample_1} satisfied.
Use $S_k^*$ to denote the returned node set. Then, if $\OPT < x$, we have $n\cdot F_{\rrsetsCon} (S_k^*) < (1 + \varepsilon^\prime) \cdot x$ with at least $1 - \delta$ probability.
\end{theorem}

\begin{proof}

\end{proof}

==> sections/lemmas/lem_sample_2.tex <==
\begin{lemma}
\label{lem:sample_2}
If $\OPT \geq x$, we have $\OPT \geq n\cdot F_{\rrsetsCon} (S_k^*) / (1 + \varepsilon^\prime)$ with probability at least $1 - \delta$.
\end{lemma}

\begin{proof}
Following the same method in the proof of Lemma \ref{lem:sample_1}, $\OPT \geq n\cdot F_{\rrsetsCon} (S_k^*) / (1 + \varepsilon^\prime)$ holds probability at least $1 - \delta$.
\end{proof}

==> sections/lemmas/lem_sample_3.tex <==
\begin{lemma}
\label{lem:sample_3}
Let $c \geq 1$. If $\OPT \geq c\cdot \frac{(1+\varepsilon^\prime)^2}{1 - 1/e - \varepsilon_1}x$, then $n\cdot F_{\rrsetsCon}(S_k^*) < (1+\varepsilon^\prime)\cdot x$ holds with at most $\delta^c$ probability.
\end{lemma}

\begin{proof}
Use $S_k^+$ to denote the size-$k$ node set that maximizes $F_{\rrsets}(S_k^+)$. By Lemma \ref{lem:guarantee_rr_size} and the properties of the greedy algorithm, we have
\begin{equation}
    F_{\rrsetsCon}(S_k^*) \geq (1-1/e-\varepsilon_1)F_{\rrsets}(S_k^+) \geq (1-1/e-\varepsilon_1)F_{\rrsets}(S_k^\circ)
\end{equation}
Let $p = \expect{F_{\rrsets}(S_k^\circ)} = \OPT / n$. From $\OPT \geq c\cdot \frac{(1+\varepsilon^\prime)^2}{1 - 1/e - \varepsilon_1}$, we have
\begin{equation}
    \begin{aligned}
    &\Pr[n\cdot F_{\rrsetsCon}(S_k^*) \leq (1 + \varepsilon^\prime)x] \\
    &\leq \Pr[n\cdot (1-1/e-\varepsilon_1)F_{\rrsets}(S_k^\circ) \leq (1 + \varepsilon^\prime)x]\\
    &\leq \Pr[n\cdot F_{\rrsets}(S_k^\circ) \leq \OPT / (1+\varepsilon^\prime)]\\
    &= \Pr[\theta_i \cdot F_{\rrsets}(S_k^\circ) - \theta_i p \leq -\varepsilon^\prime \cdot \theta_i p / (1+\varepsilon^\prime)].
    \end{aligned}
\end{equation}
By the properties of martingales,
\begin{equation}
    \Pr[\theta_i \cdot F_{\rrsets}(S_k^\circ) - \theta_i p \leq -\varepsilon^\prime \cdot \theta_i p / (1+\varepsilon^\prime)] < (\delta / {\textstyle \binom{n}{k}})^c.
\end{equation}
By the union bound, for all possible size-$k$ node set $S_k^*$, we have $n\cdot F_{\rrsetsCon}(S_k^*) \leq (1 + \varepsilon^\prime)x$ with at most $\delta^c$ probability, which completes the proof.
\end{proof}

==> sections/lemmas/lem_sample_4.tex <==
\begin{lemma}
Suppose $\rrsetsCon$ is the output of Algorithm \ref{alg:IMM_sample}. We have $\LB \geq \frac{1-1/e-\varepsilon_1}{(1+\varepsilon^\prime)^2} \OPT$ with at least $1-1/n^l$ probability.
\end{lemma}

\begin{proof}
Algorithm \ref{alg:IMM_sample} terminates before the $j$-th iteration with at least $1-1/n^l$ probability, where we have $\OPT \leq \frac{(1+\varepsilon^\prime)^2}{1 - 1/e - \varepsilon_1}x$. This gives
\[
\LB = n\cdot F_{\rrsetsCon}(S_i) / (1+\varepsilon^\prime) \geq x \geq \frac{1 - 1/e - \varepsilon_1}{(1+\varepsilon^\prime)^2}\OPT.
\]
Thus, the total number of RR sets generated in the first $j-1$ iterations is bounded by
\begin{equation}
    \max \left\{ \frac{\lambda^*}{\LB}, \frac{\lambda^\prime}{n/2^{j-1}}\right\} \leq \frac{2\max \left\{\lambda^*, \lambda^\prime\right\} \cdot (1+\varepsilon^\prime)^2}{(1-1/e-\varepsilon_1)\OPT}.
\end{equation}
Then, by the result of IMM, it is easy to prove that
\begin{equation}
    \expect{\abs{\rrsetsCon}} \leq \frac{3\max \left\{\lambda^*, \lambda^\prime\right\} \cdot (1+\varepsilon^\prime)^2}{(1-1/e-\varepsilon_1)\OPT},
\end{equation}
which gives us the upper bound of the expected number of RR sets generated by Algorithm \ref{alg:IMM_sample}.
\end{proof}

==> sections/lemmas/thm_IMA_IC_guarantee.tex <==
\begin{theorem}\label{thm:IMA_IC_guarantee}
    \color{red} Algorithm \ref{alg:IMA_IC_Acc} returns a $(\greedyFactor)$-approximate solution to the IMA problem.
\end{theorem}


==> sections/lemmas/thm_IMA_guarantee.tex <==
\begin{theorem}\label{thm:IMA_IC_guarantee_time}
    Let $\eta = \min \{\abs{\Ecand}, n\}$, and $v_m$ be the most influential node. Algorithm \ref{alg:AIS} returns a $(\greedyFactor)$-approximate solution to the IMA problem with probability $1-\delta$, running in time $O(\frac{k^2\log (k\eta /\delta)}{\varepsilon^{2} \sigma(S)} \cdot (k\sigma(\{v_m\}) + (m+n)\expect{\sigma(\{v^*\})}) + k\abs{\Ecand})$.
\end{theorem}

==> sections/lemmas/thm_IMM_sample.tex <==
\begin{theorem}
\label{thm:IMM_sample}
With at least $1-1/n^{l}$ probability, Algorithm \ref{alg:IMM_sample} returns a set $\rrsetsCon$ of size-constrained RR sets with $\abs{\rrsetsCon} \geq \lambda^* / \OPT$, where $\lambda^*$ is defined in Equation \ref{eq:params}.
\end{theorem}

\begin{proof}
When $\delta = 1 / (n^l \log_2 n)$, $\theta_i$ equals the smallest $\theta$ that satisfies equation (\ref{eq:sample_1}). 
Let $j = \myceil{\log_2 \frac{n}{\OPT}}$, which means that the corresponding $x$ the largest possible value smaller than $\OPT$ in the algorithm. By the union bound and Lemma \ref{lem:sample_1}, the probability that the algorithm terminates the loop before the $j$-th iteration is at most $\frac{j-1}{n^l \log_2 n}$. Then, by Lemma \ref{lem:sample_2} and union bound, the probability that the algorithm fails to give a lower bound of $\OPT$ is at most $\frac{j}{n^l \log_2 n}$. Since we know that $j < \log_2 n$, Algorithm \ref{alg:IMM_sample} sets $\LB \leq \OPT$ with probability at least $1 - n^{-l}$.
\end{proof}

==> sections/lemmas/thm_final.tex <==
\begin{theorem}
\label{thm:final_alg}
Given a social graph $G$, an error term $\varepsilon$, the desired size of the seed set $k$ and a parameter $l$ related to the success probability, Algorithm \ref{alg:final} will give a $(1-1/e-\varepsilon)$-approximate solution to the IM problem, with probability $1-1/n^l$.
\end{theorem}

==> sections/lemmas/thm_mc_greedy.tex <==
\begin{theorem}
    The MC-Greedy algorithm returns a $(\greedyFactor)$-approximate solution to the IMA problem with probability $1-\delta$, running in time complexity $O(\frac{k^3mn\abs{\Ecand} \log(k\abs{\Ecand}/\delta)}{\varepsilon^2})$.
\end{theorem}

\begin{proof}
As the objective function is submodular, the standard greedy algorithm provides a $(1-1/\e)$-guarantee.

To obtain a $(\greedyFactor)$-approximation ratio, we need to guarantee the Monte-Carlo estimation error $0 < \lambda \leq \frac{\varepsilon / k}{2 + \varepsilon / k}$. Let $X_1, X_2, \dots, X_r$ be $r$ independent random variables and $X_i \in [0, 1]$. Let $\bar{X} = \sum_{i=1}^{r} X_i / r$. The Chernoff bound states that, for any $\lambda \in (0, 1)$,
\begin{equation}
    \Pr[\abs{\bar{X} - \expect{\bar{X}}} \geq \lambda \expect{\bar{X}}] \leq 2\exp\left(-\frac{r\lambda^2 \expect{\bar{X}}}{3}\right).
\end{equation}
For the case of IMA, $X_i$ indicates the fraction of active nodes in the $i$-th simulation for the seed set $S$ in graph $G \cup A$, $\bar{X}$ is the returned value of Monte Carlo estimation after $r$ simulations, $\expect{\bar{X}}$ is $\sigma(A, S) / n$, and $\lambda = \frac{\varepsilon / k}{2 + \varepsilon / k}$.

We need to estimate the function for $k\abs{\Ecand}$ sets. So by the union bound, the number of simulations $r = O(\frac{n\log (k\abs{\Ecand} / \delta)}{\lambda^2}) = O(\frac{k^2 n\log (k\abs{\Ecand} / \delta)}{\varepsilon^2})$. Finally, the overall time complexity is rephrased as $O(\frac{k^3mn\abs{\Ecand} \log(k\abs{\Ecand}/\delta)}{\varepsilon^2})$.
\end{proof}

==> sections/lemmas/thm_stopping_rule.tex <==
\begin{theorem}[\cite{zhu20212}]\label{thm:stopping_rule}
    Using the RR sets returned by Algorithm \ref{alg:sample_stopping_rule}, $n\fracR{\rrsets}{S}$ is a $(\lambda, \delta)$-estimation of $\sigma(S)$.
\end{theorem}

% \begin{proof}
%     Using $X_i$ to denote a random variable indicating whether the $i$-th RR set is covered by $S$. If $R_i \cap S \neq \emptyset$, $X_i=1$. Otherwise, $X_i=0$. Then $\Sigma = \sum_{i=1}^{\theta} X_i$.

%     From the definition we know that $\Sigma / \theta = \fracR{\rrsets}{S}$, and let $p = \sigma(S) / n$. Since $X_i$ is a Bernoulli random variable, we know that when Algorithm \ref{alg:sample_stopping_rule} terminates, $\Sigma = \myceil{\Upsilon}$. Let $\nu = \frac{\myceil{\Upsilon}}{(1+\lambda) p}$.
        
%         \begin{align*}
%             &\Pr [\fracR{\rrsets}{S} > (1+\lambda) p]\\
%             &=\Pr [\myceil{\Upsilon} > (1+\lambda) p \theta]\\
%             &=\Pr [\nu > \theta] 
%             \leq \Pr \left[\sum_{i=1}^{\myfloor{\nu}} X_i + (\nu - \myfloor{\nu}X_{\myceil{\nu}}) > \sum_{i=1}^{\theta} X_i \right]\\
%             &= \Pr \left[\sum_{i=1}^{\myfloor{\nu}} X_i + (\nu - \myfloor{\nu}X_{\myceil{\nu}}) > \myceil{\Upsilon} \right]\\
%             &= \Pr \left[\frac{\sum_{i=1}^{\myfloor{\nu}} X_i + (\nu - \myfloor{\nu}X_{\myceil{\nu}})}{\nu} > \frac{\myceil{\Upsilon}}{\nu} \right]\\
%             &= \Pr \left[\frac{\sum_{i=1}^{\myfloor{\nu}} X_i + (\nu - \myfloor{\nu}X_{\myceil{\nu}})}{\nu} > (1+\lambda) p \right]\\
%             &\leq \exp \Brackets{-\frac{\lambda^2 p \nu}{2 + \frac{2}{3} \lambda}}\\
%             &= \exp \Brackets{-\frac{\lambda^2 \myceil{\Upsilon}}{2(1+\lambda)(1 + \frac{\lambda}{3})}}\\
%             &\leq \exp \Brackets{-\frac{\lambda^2 \Upsilon}{2(1+\lambda)(1 + \frac{\lambda}{3})}}\\
%             &= \frac{\delta_2}{2}.
%         \end{align*}    
        
%     Now that we have proved $\Pr [n\fracR{\rrsets}{S} > (1+\lambda) \sigma(S)] \leq \frac{\delta_2}{2}$, we can easily prove that $\Pr [n\fracR{\rrsets}{S} < (1-\lambda) \sigma(S)] \leq \frac{\delta_2}{2}$ following the same manner. Due to space limit we omit the derivation here. Hence the proof is complete.
% \end{proof}
